Cascade IPG Observer for Underwater Robot State Estimation

This paper presents a novel cascade nonlinear observer framework for inertial state estimation. It tackles the problem of intermediate state estimation when external localization is unavailable or in the event of a sensor outage. The proposed observer comprises two nonlinear observers based on a recently developed iteratively preconditioned gradient descent (IPG) algorithm. It takes the inputs via an IMU preintegration model where the first observer is a quaternion-based IPG. The output for the first observer is the input for the second observer, estimating the velocity and, consequently, the position. The proposed observer is validated on a public underwater dataset and a real-world experiment using our robot platform. The estimation is compared with an extended Kalman filter (EKF) and an invariant extended Kalman filter (InEKF). Results demonstrate that our method outperforms these methods regarding better positional accuracy and lower variance.

==> sections/draft.tex <==
%We propose a moving horizon estimation technique to localize an underwater robot. Moving Horizon Estimation is a 

% investigates the idea of iteratively preconditioned gradient-descent (IPG) to solve MHE problem with the aim of an improved performance than the existing solution techniques. To our knowledge, the preconditioning technique is used for the first time in this paper to reduce the computational cost and accelerate the crucial optimization step for MHE. The convergence guarantee of the proposed iterative approach for a class of MHE problems is presented. Additionally, sufficient conditions for the MHE problem to be convex are also derived. Finally, the proposed method is implemented on a unicycle localization example. The simulation results demonstrate that the proposed approach can achieve better accuracy with reduced computational costs.






aim is to design a discrete-time dynamical system 
to estimate the sampled system trajectory using a moving
window of the past $N$ measurements and inputs so that

the output  of the designed system is an estimate of the
system states $x_k$ in the sense that $\lim_{k \rightarrow \infty} \|x_k - \hat{x}_k \| = 0$.

For example, the observers proposed in [9], [14]–
[16] require (1)-(2) in the observer canonical form. While
this form does not lose generality in the case of observable
linear systems, for nonlinear systems only input affine
systems have been shown to be only the locally
equivalent to observer canonical form by a change of
coordinates [17]. The observers in [12] require the output
mapping h to be linear and assume the nonlinearity in F
to be either quadratically bounded or one-sided Lipschitz.
The observers in [6], [7], [13] require the output mapping
h to be linear. The observers in [4], [8], [10], [11] require
the linearity in F to be upper-triangular and h to be linear.
Compared to these vast literature, we do not restrict our
observer to any particular structures in F, h.


The performance of most of
the aforementioned observers in presence of measurement
noise has not been investigated. Process and measurement
noise in the system (1)-(2) have been considered in the
observers in [12], [24]. 

the limitation of MHE observer in [24] is
discussed in Section I-A.


Another class is the high-gain observers [15], [18]–[21]
which involves computing a robust inverse of the nonlinear
observability matrix. The observer in [15] requires (1)-(2) to
be in the observer canonical form. The observers in [21]
combine the high-gain formulation in [18] with a robust
inversion strategy, without explicitly computing the inverse
observability matrix. However, [21] requires continuous-time
measurements of the system. A unified framework of highgain
observers for uncertain systems with continuous-time
measurements is presented in [20]. We use only sampled
measurements (2), which is more practical. The qDES observer
framework developed in [22] in presence of measurement
noise includes the aforementioned exact linearizationbased
and high-gain observers among others. However,
constructing a qDES observer relies on choosing suitable
storage and class K functions so that certain conditions are
satisfied [22].

{\color{blue} 
	Copy: (to revise) 



Our proposed observer belongs to the class of Newton
and approximate Newton observers [27]–[30]. Based on the
Newton observer in [27], the finite-difference approximationbased
observer in [28] and the GMRES-based observer
in [29] are proposed for the case when, instead of (1), the
continuous-time dynamics is known. A Broyden’s methodbased
quasi-Newton observer has been proposed in [27].
However, these Newton-type observers result in large steadystate
error, even instability, when subjected to measurement
noise. 

When, instead of (1), the continuous-time dynamics is
known, an observer based on Carleman linearization-based
discretization of the continuous time-dynamics is proposed
in [31]. As shown in [31], the performance of the observer
improves with the order of truncation in the discretization,
but at the expense of computing higher order coefficients
which adds to the computational cost. In our method, 


}

Among other related works, the observer in [32] is a partial
state observer. The differential-algebraic equation-based
observer in [33], the observability function-based observer
in [34], and the observer in [35] require continuous-time
measurements of the system. We use only sampled measurements,
which is more practical. An observer for nonlinear
discrete-time dynamics (1)-(2) based on linear parameter
varying optimization is proposed in [36]. .



Hence, for showing past $N$ consecutive measurements like Eq. (4), $Y_m$ becomes
\begin{align}
	Y_{m_i} & = \left[ y_{m_{i-N+1}}, ..., y_{m_i} \right]^T \nonumber \\
	& = \begin{bmatrix}
		h(x_{m_{i-N+1}}) \\
		h \circ \Tilde{f}_{i-N+1} \\
		\vdots \\
		h \circ \Tilde{f}_{i-1} \circ \Tilde{f}_{i-2} \circ \dots \circ \Tilde{f}_{i-N+1}
	\end{bmatrix} + 
	\begin{bmatrix}
		\eta_{m_{i-N+1}} \\
		\eta_{m_{i-N+2}} \\
		\vdots \\
		\eta_{m_i}
	\end{bmatrix} \\
	& := \Tilde{H}(x_{m_{i-N+1}}, U) + W_k
\end{align}
where $\Tilde{f}$ functions (for state propagating) are calculated by
\begin{align}
	\Tilde{f}_{i-N+1} & = f(x_{j+T-1}, u_{j+T-1}) \circ \dots \circ f(x_{j+1}, u_{j+1}) \circ f(x_{j}, u_{j}), \quad j=m_{i-N+1}, \, T = m_{i-N+2} - m_{i-N+1} \\
	\Tilde{f}_{i-N+2} & = f(x_{j+T-1}, u_{j+T-1}) \circ \dots \circ f(x_{j+1}, u_{j+1}) \circ f(x_{j}, u_{j}), \quad j=m_{i-N+2}, \, T = m_{i-N+3} - m_{i-N+2} \\
	& \dots \nonumber \\
	\Tilde{f}_{i-1} & = f(x_{j+T-1}, u_{j+T-1}) \circ \dots \circ f(x_{j+1}, u_{j+1}) \circ f(x_{j}, u_{j}), \quad j=m_{i-1}, \, T = m_{i} - m_{i-1} 
\end{align}

Currently, the challenging step is to compute $\left(\frac{\partial \Tilde{H}(x_{m_{i-N+1}}, U)}{\partial x} \right)^T$ and evaluate at $w^i_{m_{i-N+1}}$. 

Comparing Eq. (10) against Eq. (7), there are a lot more intermediate steps, and in each step the control inputs can be different. Hence, it is computationally expensive to symbolically complete this step. 

\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{figures/test1_traj.png}
	\caption{}
	\label{fig:test1traj}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{figures/test1_error.png}
	\caption{}
	\label{fig:test1error}
\end{figure}


Test 2. Measurement noise:  $z_k=h(\eta_k)+\epsilon_k = (x_k+\epsilon_{1k}; y_k+\epsilon_{2k}), \epsilon_{1k}, \epsilon_{2k} \sim N(0, 0.2)$.


\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{figures/test2_error.png}
	\caption{}
	\label{fig:test2error}
\end{figure}

\FloatBarrier

\subsubsection{One observation within a few time steps}

In this section, the examples are tested when there is an observation for every few time steps. For the time steps that do not have observation values, we approximate the observations by using the last available measurements. 

In the tests, the initial states are $x_0 = [0, 0, 0]^T$. $T = 200$ or $T = 600$ is the total number of steps. $K$ is the number of time steps that contains one actual observation. The vehicle's forward speed is fixed, and at some time steps there exist the angular velocity inputs.

First, we plot the results for the cases an observation is obtained every $K=5$ time steps. The results show that the IPG approach perform slightly better than the EKF method.



Regroup the equations:
\begin{align}
	\dot{\eta} & = f_\eta(\eta) \nu \\
	\dot{\nu} & = f_\nu(\nu) + B\tau
\end{align}


\begin{align}
	\dot{x} = Ax + B\tau + d
\end{align}



In real datasets and tests, the system dynamics have a higher frequency than the observer, i.e., there are not observations in Eq.(2) at each time step. The dynamics will look like as follows,

\begin{align}
	x_{k+1} & = f(x_k, u_k), \quad k = 1, ..., K \\
	y_{m_i} & = h(x_{m_i}) + \varepsilon_{m_i}, \quad i = 1, ..., M, \quad {m_i} \in \{ 1, ..., K\} %\begin{cases}
	%\{ \} & \quad \text{when no observation} \\
	%h(x_m) + \varepsilon_m & \quad \text{when observed}
	%\end{cases}
\end{align}
